DotFAN: A Domain-transferred Face Augmentation Network for Pose and Illumination Invariant Face Recognition

The performance of a convolutional neural network (CNN) based face recognition model largely relies on the richness of labelled training data. Collecting a training set with large variations of a face identity under different poses and illumination changes, however, is very expensive, making the diversity of within-class face images a critical issue in practice. In this paper, we propose a 3D model-assisted domain-transferred face augmentation network (DotFAN) that can generate a series of variants of an input face based on the knowledge distilled from existing rich face datasets collected from other domains. DotFAN is structurally a conditional CycleGAN but has two additional subnetworks, namely face expert network (FEM) and face shape regressor (FSR), for latent code control. While FSR aims to extract face attributes, FEM is designed to capture a face identity. With their aid, DotFAN can learn a disentangled face representation and effectively generate face images of various facial attributes while preserving the identity of augmented faces. Experiments show that DotFAN is beneficial for augmenting small face datasets to improve their within-class diversity so that a better face recognition model can be learned from the augmented dataset.

==> facebib.tex <==
@article{chawla2002smote,
  title={SMOTE: Synthetic minority over-sampling technique},
  author={Chawla, N. V. and Bowyer, K. W. and Hall, L. O. and Kegelmeyer, W. P.},
  journal={J. Artificial Intell. Research},
  volume={16},
  pages={321--357},
  year={2002}
}

@article{zhang2018face,
  title={Face Frontalization Using an Appearance-Flow-Based Convolutional Neural Network},
  author={Zhang, Z. and Chen, X. and Wang, B. and Hu, G. and Zuo, W. and Hancock, E. R.},
  journal={IEEE Trans. Image Process.},
  volume={28},
  number={5},
  pages={2187--2199},
  year={2018},
  publisher={IEEE}
}
@inproceedings{shen2017learning,
  title={Learning residual images for face attribute manipulation},
  author={Shen, W. and Liu, R.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={4030--4038},
  year={2017}
}
@article{radford2015unsupervised,
  title={Unsupervised representation learning with deep convolutional generative adversarial networks},
  author={Radford, A. and Metz, L. and Chintala, S.},
  journal={arXiv preprint arXiv:1511.06434},
  year={2015}
}
@inproceedings{li2018beautygan,
  title={Beautygan: Instance-level facial makeup transfer with deep generative adversarial network},
  author={Li, T. and Qian, R. and Dong, C. and Liu, S. and Yan, Q. and Zhu, W. and Lin, L.},
  booktitle={Proc. ACM Multimedia},
  pages={645--653},
  year={2018},
}
@inproceedings{lu2018attribute,
  title={Attribute-guided face generation using conditional {CycleGAN}},
  author={Lu, Y. and Tai, Y.-W. and Tang, C.-K.},
  booktitle={Proc. European Conf.  Comput. Vis.},
  pages={282--297},
  year={2018}
}

@inproceedings{cui2019class,
  title={Class-balanced loss based on effective number of samples},
  author={Cui, Y. and Jia, M. and Lin, T.-Y. and Song, Y. and Belongie, S.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={9268--9277},
  year={2019}
}

@inproceedings{szegedy2016rethinking,
  title={Rethinking the inception architecture for computer vision},
  author={Szegedy, C. and Vanhoucke, V. and Ioffe, S. and Shlens, J. and Wojna, Z.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={2818--2826},
  year={2016}
}

@inproceedings{blanz1999morphable,
  title={A morphable model for the synthesis of {3D} faces.},
  author={Blanz, V. and Vetter, T. and others},
  booktitle={Proc. ACM SIGGRAPH},
  year={1999}
}

@inproceedings{choi2018stargan,
  title={Stargan: Unified generative adversarial networks for multi-domain image-to-image translation},
  author={Choi, Y. and Choi, M. and Kim, M. and Ha, J.-W. and Kim, S. and Choo, J.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={8789--8797},
  year={2018}
}
@inproceedings{liu2015deep,
  title={Deep learning face attributes in the wild},
  author={Liu, Z. and Luo, P. and Wang, X. and Tang, X.},
  booktitle={Proc. IEEE Int. Conf. Comput. Vis.},
  pages={3730--3738},
  year={2015}
}
@article{yi2014learning,
  title={Learning face representation from scratch},
  author={Yi, D. and Lei, Z. and Liao, S. and Li, S. Z.},
  journal={arXiv preprint arXiv:1411.7923},
  year={2014}
}
@inproceedings{kinga2015method,
	title={A method for stochastic optimization},
	author={Kinga, D. and Adam, J. B.},
	booktitle={Proc. Int. Conf. Learn. Represent.},
	volume={5},
	year={2015}
}
@inproceedings{guo2016ms,
  title={{MS-celeb}-1m: A dataset and benchmark for large-scale face recognition},
  author={Guo, Y. and Zhang, L. and Hu, Y. and He, X. and Gao, J.},
  booktitle={Proc. European Conf. Comput. Vis.},
  pages={87--102},
  year={2016},
}
@article{howard2017mobilenets,
  title={Mobilenets: Efficient convolutional neural networks for mobile vision applications},
  author={Howard, A. G. and Zhu, M. and Chen, B. and Kalenichenko, D. and Wang, W. and Weyand, T. and Andreetto, M. and Adam, H.},
  journal={arXiv preprint arXiv:1704.04861},
  year={2017}
}
@inproceedings{dai2016instance,
  title={Instance-aware semantic segmentation via multi-task network cascades},
  author={Dai, J. and He, K. and Sun, J.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={3150--3158},
  year={2016}
}
@article{gross2010multi,
  title={Multi-pie},
  author={Gross, R.and Matthews, I. and Cohn, J. and Kanade, T. and Baker, S.},
  journal={Image Vis. Comput.},
  volume={28},
  number={5},
  pages={807--813},
  year={2010},
}
@inproceedings{hassner2015effective,
  title={Effective face frontalization in unconstrained images},
  author={Hassner, T. and Harel, S. and Paz, E. and Enbar, R.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={4295--4304},
  year={2015}
}
@article{mirza2014conditional,
  title={Conditional generative adversarial nets},
  author={Mirza, M. and Osindero, S.},
  journal={arXiv preprint arXiv:1411.1784},
  year={2014}
}
@inproceedings{mejjati2018unsupervised,
  title={Unsupervised attention-guided image-to-image translation},
  author={Mejjati, Y. A. and Richardt, C. and Tompkin, J. and Cosker, D. and Kim, K. I.},
  booktitle={Proc. Adv. Neural Inf. Proc. Syst.},
  pages={3693--3703},
  year={2018}
}
@inproceedings{zhou2019deep,
  title={Deep Single-Image Portrait Relighting},
  author={Zhou, Hao and Hadap, Sunil and Sunkavalli, Kalyan and Jacobs, David W},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={7194--7202},
  year={2019}
}
@inproceedings{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, I. and Pouget-Abadie, J. and Mirza, M. and Xu, B. and Warde-Farley, D. and Ozair, S. and Courville, A. and Bengio, Y.},
  booktitle={Proc. Adv. Neural Inf. Proc. Syst.},
  pages={2672--2680},
  year={2014}
}
@inproceedings{zhu2017unpaired,
  title={Unpaired image-to-image translation using cycle-consistent adversarial networks},
  author={Zhu, J.-Y. and Park, T. and Isola, P. and Efros, A. A.},
  booktitle={Pro. IEEE Int. Conf. Comput. Vis.},
  pages={2223--2232},
  year={2017}
}
@inproceedings{zhu2015high,
  title={High-fidelity pose and expression normalization for face recognition in the wild},
  author={Zhu, X. and Lei, Z. and Yan, J. and Yi, D. and Li, S. .Z},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={787--796},
  year={2015}
}
@inproceedings{isola2017image,
  title={Image-to-image translation with conditional adversarial networks},
  author={Isola, P. and Zhu, J.-Y. and Zhou, T. and Efros, A. A.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={1125--1134},
  year={2017}
}
@inproceedings{deng2019arcface,
  title={Arcface: Additive angular margin loss for deep face recognition},
  author={Deng, J. and Guo, J. and Xue, N. and Zafeiriou, S.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={4690--4699},
  year={2019}
}
@inproceedings{sengupta2016frontal,
  title={Frontal to profile face verification in the wild},
  author={Sengupta, S. and Chen, J.-C. and Castillo, C. and Patel, V. M. and Chellappa, R. and Jacobs, D. W.},
  booktitle={Proc. IEEE Winter Conf. Appl. Comput. Vis.},
  pages={1--9},
  year={2016},
}
@inproceedings{huang2008labeled,
  title={Labeled faces in the wild: A database forstudying face recognition in unconstrained environments},
  author={Huang, G. B. and Mattar, M. and Berg, T. and Learned-Miller, E.},
  year={2008}
}
@inproceedings{chen2016unconstrained,
  title={Unconstrained face verification using deep cnn features},
  author={Chen, J.-C. and Patel, V. M. and Chellappa, R.},
  booktitle={Proc. IEEE Winter Conf. Appl. Comput. Vis.},
  pages={1--9},
  year={2016},
}
@inproceedings{klare2015pushing,
  title={Pushing the frontiers of unconstrained face detection and recognition: Iarpa janus benchmark a},
  author={Klare, B. F. and Klein, B. and Taborsky, E. and Blanton, A. and Cheney, J. and Allen, K. and Grother, P. and Mah, A. and Jain, A. K.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={1931--1939},
  year={2015}
}
@inproceedings{chen2018mobilefacenets,
  title={Mobilefacenets: Efficient {CNNs} for accurate real-time face verification on mobile devices},
  author={Chen, S. and Liu, Y. and Gao, X. and Han, Z.},
  booktitle={Proc. Chinese Conf. Biometric Recognit.},
  pages={428--438},
  year={2018},
}

@inproceedings{gulrajani2017improved,
  title={Improved training of {Wasserstein GANs}},
  author={Gulrajani, I. and Ahmed, F. and Arjovsky, M. and Dumoulin, V. and Courville, A. C.},
  booktitle={Proc. Adv. Neural Inf. Proc. Syst.},
  pages={5767--5777},
  year={2017}
}
@inproceedings{zhu2016face,
  title={Face alignment across large poses: A {3D} solution},
  author={Zhu, X. and Lei, Z. and Liu, X. and Shi, H. and Li, S. Z.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={146--155},
  year={2016}
}
@inproceedings{qian2019unsupervised,
  title={Unsupervised Face Normalization With Extreme Pose and Expression in the Wild},
  author={Qian, Y. and Deng, W. and Hu, J.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={9851--9858},
  year={2019}
}
@inproceedings{cole2017synthesizing,
  title={Synthesizing normalized faces from facial identity features},
  author={Cole, F. and Belanger, D. and Krishnan, D. and Sarna, A. and Mosseri, I. and Freeman, W. T.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={3703--3712},
  year={2017}
}
@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, K. and Zhang, X. and Ren, S. and Sun, J.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={770--778},
  year={2016}
}
@inproceedings{wang2018cosface,
  title={{CosFace}: Large margin cosine loss for deep face recognition},
  author={Wang, H. and Wang, Y. and Zhou, Z. and Ji, X. and Gong, D. and Zhou, J. and Li, Z. and Liu, W.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={5265--5274},
  year={2018}
}
@article{wang2018deep,
  title={Deep face recognition: A survey},
  author={Wang, M. and Deng, W.},
  journal={arXiv preprint arXiv:1804.06655},
  year={2018}
}
@inproceedings{finlayson2002removing,
  title={Removing shadows from images},
  author={Finlayson, G. D. and Hordley, S. D. and Drew, M. S.},
  booktitle={Proc. European Conf. Comput. Vis.},
  pages={823--836},
  year={2002},
}
@article{jobson1997multiscale,
  title={A multiscale retinex for bridging the gap between color images and the human observation of scenes},
  author={Jobson, D. J. and Rahman, Z. and Woodell, G. A.},
  journal={IEEE Trans. Image Proc.},
  volume={6},
  number={7},
  pages={965--976},
  year={1997},
}
@article{land1971lightness,
  title={Lightness and retinex theory},
  author={Land, E. H. and McCann, J. J.},
  journal={Josa},
  volume={61},
  number={1},
  pages={1--11},
  year={1971},
  publisher={Optical Society of America}
}
@article{wang2008face,
  title={Face relighting from a single image under arbitrary unknown lighting conditions},
  author={Wang, Y. and Zhang, L. and Liu, Z. and Hua, G. and Wen, Z. and Zhang, Z. and Samaras, D.},
  journal={IEEE Trans. Pattern Anal. Mach. Intell.},
  volume={31},
  number={11},
  pages={1968--1984},
  year={2008},
}
@article{jiang2005efficient,
  title={Efficient {3D} reconstruction for face recognition},
  author={Jiang, D. and Hu, Y. and Yan, S. and Zhang, L. and Zhang, H. and Gao, W.},
  journal={Pattern Recognit.},
  volume={38},
  number={6},
  pages={787--798},
  year={2005},
}
@inproceedings{yin2017towards,
  title={Towards large-pose face frontalization in the wild},
  author={Yin, X. and Yu, X. and Sohn, K. and Liu, X. and Chandraker, M.},
  booktitle={Proc. IEEE Int. Conf. Comput. Vis.},
  pages={3990--3999},
  year={2017}
}
@inproceedings{huang2017beyond,
  title={Beyond face rotation: Global and local perception {GAN} for photorealistic and identity preserving frontal view synthesis},
  author={Huang, R. and Zhang, S. and Li, T. and He, R.},
  booktitle={Proc. IEEE Int. Conf. Comput. Vis.},
  pages={2439--2448},
  year={2017}
}
@inproceedings{zhao2018towards,
  title={Towards pose invariant face recognition in the wild},
  author={Zhao, J. and Cheng, Y. and Xu, Y. and Xiong, L. and Li, J. and Zhao, F. and Jayashree, K. and Pranata, S. and Shen, S. and Xing, J. and others},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={2207--2216},
  year={2018}
}
@inproceedings{tran2017disentangled,
  title={Disentangled representation learning {GAN} for pose-invariant face recognition},
  author={Tran, L. and Yin, X. and Liu, X.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={1415--1424},
  year={2017}
}
@inproceedings{hu2018pose,
  title={Pose-guided photorealistic face rotation},
  author={Hu, Y. and Wu, X. and Yu, B. and He, R. and Sun, Z.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={8398--8406},
  year={2018}
}

@inproceedings{shen2018faceid,
  title={{FaceID-GAN}: Learning a symmetry three-player {GAN} for identity-preserving face synthesis},
  author={Shen, Y. and Luo, P. and Yan, J. and Wang, X. and Tang, X.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={821--830},
  year={2018}
}
@inproceedings{cao2018pose,
  title={Pose-robust face recognition via deep residual equivariant mapping},
  author={Cao, K. and Rong, Y. and Li, C. and Tang, X. and Loy, C. C.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={5187--5196},
  year={2018}
}
@inproceedings{masi2016pose,
  title={Pose-aware face recognition in the wild},
  author={Masi, I. and Rawls, S. and Medioni, G. and Natarajan, P.},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={4838--4846},
  year={2016}
}

